Estimation and Validation of Ratio-based Conditional Average Treatment Effects Using Observational Data

While sample sizes in randomized clinical trials are large enough to estimate the average treatment effect well, they are often insufficient for estimation of treatment-covariate interactions critical to studying data-driven precision medicine. Observational data from real world practice may play an important role in alleviating this problem. One common approach in trials is to predict the outcome of interest with separate regression models in each treatment arm, and estimate the treatment effect based on the contrast of the predictions. Unfortunately, this simple approach may induce spurious treatment-covariate interaction in observational studies when the regression model is misspecified. Motivated by the need of modeling the number of relapses in multiple sclerosis patients, where the ratio of relapse rates is a natural choice of the treatment effect, we propose to estimate the conditional average treatment effect (CATE) as the ratio of expected potential outcomes, and derive a doubly robust estimator of this CATE in a semiparametric model of treatment-covariate interactions. We also provide a validation procedure to check the quality of the estimator on an independent sample. We conduct simulations to demonstrate the finite sample performance of the proposed methods, and illustrate their advantages on real data by examining the treatment effect of dimethyl fumarate compared to teriflunomide in multiple sclerosis patients.

==> survival.tex <==
In precision medicine, many clinically meaningful outcomes to are time-to-event outcomes. For example, among MS patients in the NTD registry, a useful endpoint to measure effectiveness is the time to first relapse. In this case, the observed training data consist of $\{(X_i, \Delta_i, R_i, Z_i), i=1,\cdots, n\},$ where $X_i=T_i\wedge C_i,$ $\Delta_i=I(T_i<C_i),$ $T_i$ is the event time of interest and $C_i$ is the censoring time. As previously, we will use $T_i^{(r)}$ and $C^{(r)}_i$ to refer to the potential event time and censoring time under treatment $r$. For time-to-event outcomes, the heterogeneous treatment effect often cannot be measured by a contrast of the conditional expectations $\E(T^{(r)}|Z=z),$ because this expectation may not be identifiable due to right censoring preventing observation of the event time beyond some maximum study length time. The parameter closest to the mean survival time that is identifiable is the restricted mean survival time, i.e., $E(T\wedge \tau)$, for an appropriate choice of $\tau > 0$. The ATE (and CATE) of the restricted mean survival time is an appropriate contrast that we can estimate with data. 

It is a popular practice to employ Cox proportional hazards model to analyze time-to-event outcomes. Let $\lambda_r(t \mid z) $ %= \lim_{h \to 0^+} \tfrac{1}{h}P(T^{(r)} \in [t,t+h) \mid Z=z, T \ge t)$ 
be the hazard function of $T_i^{(r)} \mid Z_i=z$, $r=0, 1.$ The Cox proportional hazards model assumes that $$\lambda_r(t \mid z)=\lambda_{r0}(t)\exp(\beta^\top_rz),$$
for $\lambda_{r0}(\cdot)$, an unspecified baseline hazard function in group $r$. In this case, $\exp\{(\beta_1-\beta_0)^\top z\}$ is a natural measure of the CATE. If the proportional hazards assumption is violated, we can still define $\beta_r$ as the root of the limit of the score equation of the Cox model.
%$$ \E \left\{ \Delta_i^{(r)}\left[Z_i-\frac{s^{(r)}_1(X_i^{(r)}; \beta)}{s_0^{(r)}(X_i^{(r)}; \beta)}\right]\right\}=0,$$
%where $(X^{(r)}, \Delta^{(r)})$ is the potential observation $(X, \Delta),$ if the patient receives treatment $r,$ and $s_j^{(r)}(t; \beta)=\E\left[Z^j \exp(\beta^\top Z)I(X^{(r)}\ge t)\right]$ \citep{lin1989robust}.
However, in this case, $\exp\{(\beta_1-\beta_0)^\top z\}$ may no longer be a sensible surrogate for the CATE even if the two arms have the same covariate distribution, as it may introduce spurious heterogeneity not present in real data. 
We provide an example in the Supplement.

In this section, we propose to use the ratio of restricted mean time lost (RMTL) due to the first relapse to measure the treatment effect, i.e.,
$$D(z)=\frac{\E\{\tau-(T^{(1)}\wedge \tau)|Z=z\}}{\E\{\tau-(T^{(0)}\wedge \tau) \mid Z=z\}},$$
where $\tau>0$ is a chosen constant \citep{uno2014moving}, since it is expected to be concordant with the relapse rate ratio. When the relapse rate is low, this ratio is similar to the hazard ratio.

To approximate this CATE, we consider the score 
$\exp\{(\beta_1-\beta_0)^\top \widetilde{z}\}$, where $\beta_r$ is the root of the the equation
$$\E\left[\widetilde Z\left\{\E(\tau-T^{(r)}\wedge \tau \mid Z)- \exp(\beta_r^\top\widetilde{Z})\right\}\right]=0.$$
While this regression model is not always natural for arbitrary choices of $\tau$, it can still be a useful working model. For example, when $T^{(r)} \mid Z=z$ follows an exponential distribution with the failure rate of $\beta_r^\top \widetilde{z}$ and $\tau$ is large relative to $\beta_r^\top \widetilde{Z}$, this model is approximately correctly specified.
Luckily, like the Poisson regression model discussed above, this approach is robust to mis-specification of the model in the sense that it doesn't introduce spurious treatment effect heterogeneity.  Therefore, it remains a useful working model for estimating heterogeneous treatment effects measured by RMTL ratio.

Again, we propose two approaches for approximating $D(z)$. In the first approach, we estimate $\beta_r$ by solving the  estimating equation based on cross-fitting:
$$n^{-1}\sum_{k=1}^K\sum_{i\in {\cal I}_k} \widetilde {Z_i}\left[\widetilde{\mu}^{(-k)}_r(Z_i, \tau)- \exp(\beta_r^\top\widetilde{Z}_i)\right]=0,$$
where $\widetilde{\mu}_r^{(-k)}(z; \tau)$ is an estimator of $E(\tau-T^{(r)}\wedge\tau \mid Z=z)$ constructed via the following step
\begin{enumerate}
    \item Construct an initial estimator of $\E(\tau-T_i^{(r)}\wedge \tau|Z_i=z)$ based on observations not in ${\cal I}_k.$
    denote the estimator by  $\what{\mu}_r^{(-k)}(z; \tau).$
    \item Solving weighted estimating equations
    $$\sum_{i \notin {\cal I}_k} \what{L}_i(r)\what{W}^{(-k)}_{i}(r) \widetilde{Z}_i\left[(\tau-T_i\wedge\tau)-\exp\left\{\alpha_r\times\log(\widehat{\mu}_r^{(-k)}(Z_i, \tau))+\gamma_r^\top \widetilde{Z}_i\right\}\right]=0, $$
    and denote the roots by $(\widehat{\alpha}_r^{(-k)}, \widehat{\gamma}_r^{(-k)\top})^\top, r=0, 1.$ 
    \item Let $\widetilde{\mu}_r^{(-k)}(z; \tau)=\exp\left\{\widehat{\alpha}_r^{(-k)}\times\log(\widehat{\mu}_r^{(-k)}(Z_i, \tau))+\widehat{\gamma}_r^{(-k)\top} \widetilde{Z}_i\right\}.$
\end{enumerate}
In the second step of constructing $\widetilde{\mu}_r^{(-k)}(\cdot, \tau)$, 
$$\what{L}_i(r)=\frac{I(T_i\wedge \tau<C_i)}{\what{K}_{Cr}(T_i\wedge \tau \mid Z_i)}$$
and 
$$\what{W}_i^{(-k)}(r)=r\frac{R_i}{\what{\pi}_1^{(-k)}(Z_i)}+(1-r)\frac{1-R_i}{\what{\pi}_0^{(-k)}(Z_i)},$$
where $I(T_i\wedge \tau<C_i)=\Delta_i+(1-\Delta_i)I(X_i\ge\tau),$ and $\what{K}_{Cr}(\cdot \mid z)$ is an estimator of the survival function of the censoring time $C_i^{(r)} \mid Z_i=z$ under a regression model, such as the Cox model. The key assumption here is that the inverse probability weighting via $\what{L}_i(r)$ can correct the effect of right censoring, as long as $\what{K}_{Cr}(t\mid z)$ is a consistent estimator of the survival function of the censoring time $C^{(r)}$ given $Z=z$ and $P(C^{(r)}>\tau|Z=z)\ge \epsilon_\tau>0.$ Let the resulting estimator of $\beta_r$ be denoted by $\what{\beta}_r$ and $D(z)$ can be approximated by 
$\exp\left\{\what{\beta}_1-\what{\beta}_0)^\top \widetilde{z}\right\}.$

\begin{remark}
The initial estimator $\what{\mu}_r^{(-k)}(z; \tau)$ can be based on any sensible regression models characterizing the relationship between $T_i^{(r)}$ and $Z_i.$  For example, one may employ the standard Cox model $\lambda_r(t \mid z)=\lambda_{r0}(t)\exp\{\eta^\top_r B(z)\}.$
%$$ \log[-\log\{S_r(t|z)\}]=\log[-\log\{S_{r0}(t)\}]+\eta^\top_rB(z);$$
%where $S_r(t|z)$ is the survival function of $T^{(r)}|Z=z.$ 
Under this model,
$$\tau-\int_0^\tau \exp\left[-\what{\Lambda}_{r0}(t)\exp\{\what\eta_r^\top B(z)\}\right]dt$$
can be used to approximate $\E(\tau-T_i^{(r)}\wedge \tau|Z_i=z)$, 
where $\what{\Lambda}_{r0}(t)$ is the Breslow estimator for the cumulative baseline hazard function and $\what{\eta}_r$ is the maximum partial likelihood estimator for $\eta_r$ in arm $r$ \citep{cheng1998prediction}.
Alternatively, we may assume a regression model tailored for restricted mean survival time \citep{tian2013predicting}:
$$\E(T^{(r)}\wedge\tau |Z=z)=\tau \frac{\exp\{\eta_r^\top B(z)\}}{1+\exp\{\eta_r^\top B(z)\}}$$
and estimate $\eta_r$ by solving the simple estimating equation
$$\sum_{i=1}^n I(R_i=r)\what{L}_i(r)B(Z_i)\left\{T_i\wedge \tau-\tau \frac{\exp\{\eta_r^\top B(Z_i)\}}{1+\exp\{\eta_r^\top B(Z_i)\}}\right\}=0.$$
Under this model, $\E(\tau-T_i^{(r)}\wedge \tau|Z_i=z)$  can be approximated by 
$$ \frac{\tau}{1+\exp\{\what{\eta}_r^\top B(z)\}},$$
where $\what{\eta}_r$ is the root to the estimating equation above. 
\end{remark}

In the second approach, we may directly estimate $\delta_0$ under the assumption that $D(z)=\exp(\delta_0^\top \widetilde{z}).$ Specifically, we estimate $\delta_0$ by solving the estimating equation by cross-fitting 
\begin{align*}
     &n^{-1}\sum_{k=1}^K\sum_{i\in {\cal I}_k} \what{L}_i(R_i)\left(\widetilde{Z}_i R_i \frac{\left[(\tau-T_i\wedge\tau)-e^{\delta^\top \widetilde{Z}_i}\widehat{\mu}^{(-k)}_0(Z_i; \tau)\right]}{e^{\delta^\top \widetilde{Z}_i}\widehat{\pi}_1^{(-k)}(Z_i)+\widehat{\pi}_0^{(-k)}(Z_i)}\widehat{\pi}_0^{(-k)}(Z_i) \right.\\
    & \left.~~~~~~~~~~~~~~~~~~~~~~~~~-\widetilde{Z}_i(1-R_i)\frac{\left[(\tau-T_i\wedge\tau)-\widehat{\mu}^{(-k)}_0(Z_i; \tau)\right]e^{\delta^\top \widetilde{Z}_i}}{e^{\delta^\top \widetilde{Z}_i}\widehat{\pi}_1^{(-k)}(Z_i)+\widehat{\pi}_0^{(-k)}(Z_i)}\widehat{\pi}_1^{(-k)}(Z_i)\right)=0,
\end{align*}
or the counterpart of $\bar{S}_n^{(cf)}(\delta)=0.$  Let the root of the equation be $\what{\delta}.$ Similar to the count outcome, $\what{\delta}$ is a consistent estimator of $\delta_0$, if either the propensity score estimator $\what{\pi}_1(z)$ or the outcome predictions $ \what{\mu}_0^{(-k)}(z; \tau)$ is consistent. However, $\what{K}_{Cr}(z)$ must be consistent, either way, to appropriately adjust for censoring using the weights $\what{L}_i(R_i).$ Then, $D(z)$ is approximately $\exp\left(\what{\delta}^\top \widetilde{z}\right).$

With an estimator $\what{D}(z)$ of the CATE, we need to estimate 
$$ AD(c)=\frac{\E\{\tau-T^{(1)}\wedge\tau|\what{D}(Z)\ge c\}}{\E\{\tau-T^{(0)}\wedge \tau| \what{D}(Z)\ge c\}}$$
based on validation data. To this end, 
%we may also construct a double robust estimator by solving the estimating equation
%\begin{align*}
%    \bar{S}^V_c(\alpha)=&\sum_{\what{D}(Z_i^V)\ge c} \what{L}^V_{ci}(R_i^V)\left(  R_i^V\left[Y_i^V-\frac{e^{\alpha}\widehat{\mu}_{c0}(Z_i^V)+\widehat{\mu}_{c1}(Z_i^V)}{2}\right]\frac{1-\what{\pi}^V_{c1}(Z_i^V)}{e^{\alpha}\what{\pi}_{c1}(Z_i^V)+(1-\what{\pi}_{c1}(Z_i^V))} \right.\\
%    &\left.- (1-R_i^V)\left[Y_i^Ve^{\alpha}-\frac{e^{\alpha}\widehat{\mu}_{c0}(Z^V_i)+\widehat{\mu}_{c1}(Z_i^V)}{2}\right]\frac{\what{\pi}_{c1}(Z_i^V)}{e^{\alpha}\what{\pi}_{c1}(Z_i^V)+(1-\what{\pi}_{c1}(Z_i^V))}\right)\\
%    =&0,
%\end{align*}
%where $\what{L}^V_{ci}(r)$ is the counterpart of $\what{L}_i(r)$ based on 
%$$ \sum_{\what{D}(Z_i^V)\ge c} \frac{I(T^V_i\wedge \tau<C^V_i)}{\what{K}_{Cr}^{V}(T_i^V\wedge \tau\mid Z_i, c)}\left(\begin{array}{c} R_i^V \\ B(Z_i^V) \\ \what{L}_i^V \end{array}\right)\left[ (\tau-T_i^V)\vee 0 -\exp\left\{\alpha R_i^V+\xi^\top B(Z_i^V)+\gamma \what{L}_i^V\right\}\right]=0$$
%for $(\alpha, \xi^\top, \gamma)^\top$,
%where $\what{K}^{V}_{Cr}(\cdot \mid z, c)$ is a estimator of the probability $P(C^V\ge t| R^V=r, Z_i^V=z)$ %. To reduce the risks of mis-specification of $\what{K}^{V}_{Cr}(\cdot \mid z,c)$, we recommend estimating it 
%using 
%only observations in the subgroup $\{Z^V \mid \what{D}(Z^V)\ge c\}$. Recall that we use the superscript $V$ to denote membership in the validation sample. The resulting root denoted by $\what{\alpha}=\what{AD}(c),$ is a double robust estimator of the ATE in the subgroup of patients. %{\red what is $V$ in all the above equations?}
we may estimate the $AD(c)$ by constructing doubly robust estimators for
$\E(\tau-T^{(r)}\wedge\tau |\what{D}(Z)\ge c), r=0, 1.$ To this end, we may construct an initial estimator for 
$\mu_r(z, \tau)=\E(\tau-T^{(r)}\wedge \tau |Z=z)$ using observations in the subgroup $\{z^V \mid \what{D}(z^V)\ge c\}$. Methods described in Remark 5 can be used to achieve this objective.   Denote the resulting estimator by $\what\mu_{cr}(z; \tau).$ We may estimate $\E(\tau-T^{(r)}\wedge\tau |\what{D}(Z)\ge c)$  by
$$m_c^{-1}\sum_{\what{D}(Z_i^V)\ge c} \left[\what{\mu}_{cr}(Z_i^V, \tau)+\what{L}_{ci}^V(r)\what{W}_{ci}^V(r)\left\{(\tau-T_i^V\wedge\tau)-\what{\mu}_{cr}(Z_i^V, \tau)\right\}\right] .$$
%\begin{align*}
%&\what\mu_r(c; \tau)=\\
%&\frac{1}{m_c}\sum_{\what{D}(R_i^V)\ge c} \left[\tau\frac{\exp(\what\eta_r(c)^\top B(Z_i^V))}{1+\exp(\what\eta_r(c)^\top B(Z_i^V))}+\what{L}_{ir}^C\frac{I(T^V_i\wedge \tau<C^V_i)}{\what{K}^{V}_{Cr}(T_i^V\wedge \tau \mid Z_i, c)}\left\{T_i\wedge\tau-\tau\frac{\exp(\what\eta_r(c)^\top B(Z_i^V))}{1+\exp(\what\eta_r(c)^\top B(Z_i^V))}\right\}  \right],
%\end{align*}
%where $m_c$ is the sample size of the subgroup $\{Z\mid \what{D}(Z)\ge c\}$ in the validation set. 
Then, we propose to estimate $AD(c)$ by the plugin estimator
$$\frac{\what\mu_1(c; \tau)}{\what\mu_0(c; \tau)}.$$
